When Generative Replay Meets Evolving Deepfakes: Dual Confusion-Aware Regularization for Incremental Face Forgery Detection

The rapid advancement of face generation techniques has introduced an increasing variety of forgery methods, making incremental deepfake detection essential for maintaining robust detectors. While generative replay provides a promising solution to alleviate catastrophic forgetting without storing historical data, its effectiveness is hindered by \textbf{domain confusion} between generated samples and real data. We observe that replay samples fall into two categories: when the replay generator closely resembles the newly introduced forgery model, generated real samples overlap with the fake domain and become \textbf{domain-risky}; when the generator differs significantly, generated samples maintain clearer domain separation and can be treated as \textbf{domain-safe}. To address this challenge, we propose a Dual \textbf{C}onfusion-\textbf{A}ware \textbf{RE}gularization strategy, termed \textbf{Dual-CARE}. A Domain-aware Confusion Score (DC Score) is introduced to quantify domain confusion and \textbf{dual-modulate} the optimization of both replay generators and the incremental detector. Guided by DC Score, replay generators are updated to better approximate previous-task distributions, while the detector adopts different supervision strategies: domain-safe samples are directly supervised, whereas domain-risky samples are regulated using a Relative Separation Loss to balance supervision and confusion. Extensive experiments demonstrate that Dual-CARE effectively exploits generative replay and improves incremental deepfake detection under evolving forgery scenarios.

==> AAAI2027/sec/0_abstract.tex <==
\begin{abstract}
The rapid advancement of face generation techniques has led to a growing variety of forgery methods. Incremental forgery detection aims to gradually update existing models with new forgery data, yet current sample replay–based methods are limited by low diversity and privacy concerns. Generative replay offers a potential solution by synthesizing past data, but its feasibility for forgery detection remains unclear. In this work, we systematically investigate generative replay and identify two scenarios: when the replay generator closely resembles the new forgery model, generated real samples blur the domain boundary, creating \textbf{domain-risky} samples; when the replay generator differs significantly, generated samples can be safely supervised, forming \textbf{domain-safe} samples. To exploit generative replay effectively, we propose a novel Domain-Aware Relative Weighting (DARW) strategy. DARW directly supervises domain-safe samples while applying a Relative Separation Loss to balance supervision and potential confusion for domain-risky samples. A Domain Confusion Score dynamically adjusts this tradeoff according to sample reliability. Extensive experiments demonstrate that DARW consistently improves incremental learning performance for forgery detection under different generative replay settings and alleviates the adverse impact of domain overlap.
\end{abstract}

==> AAAI2027/tab/alpha_p1.tex <==
\begin{table*}[h!]
\centering
\caption{Ablation study of normalization functions for the DC Score ($\alpha$) under Protocol 1.}
\footnotesize
\begin{tabular}{l@{\hspace{3pt}} c | c c c c c c c c}
\toprule
Method & Task & LDM & DFDCP & SDv21 & DDPM & DiT & CDF & Avg. & $\alpha$ \\
\toprule

% ================== OURS tanh ==================
\multirow{6}{*}{tanh}
& T1 & 99.99 & - & - & - & - & - & 99.99 & - \\
& T2 & 99.90 & 91.50 & - & - & - & - & 95.70 & 93.86 \\
& T3 & 99.78 & 95.01 & 99.96 & - & - & - & 98.25 & 99.82 \\
& T4 & 98.95 & 92.73 & 97.41 & 99.99 & - & - & 97.27 & 25.99 \\
& T5 & 98.62 & 85.14 & 97.40 & 97.62 & 99.24 & - & 95.60 & 93.25 \\
& T6 & 99.69 & 89.07 & 98.39 & 99.47 & 88.29 & 99.51 & 95.74 & 99.36 \\
\midrule

% ================== sigmoid ==================
\multirow{6}{*}{sigmoid}
& T1 & 99.99 & - & - & - & - & - & 99.99 & - \\
& T2 & 99.94 & 90.98 & - & - & - & - & 95.46 & 82.49 \\
& T3 & 99.91 & 94.89 & 99.92 & - & - & - & 98.24 & 98.15 \\
& T4 & 99.04 & 93.40 & 98.77 & 99.99 & - & - & 97.80 & 74.07 \\
& T5 & 98.36 & 90.01 & 94.45 & 97.82 & 96.72 & - & 95.47 & 77.36 \\
& T6 & 92.79 & 87.27 & 96.59 & 99.49 & 85.42 & 99.60 & 93.53 & 92.20 \\
\midrule

% ================== d/5 ==================
\multirow{6}{*}{d/5}
& T1 & 99.99 & - & - & - & - & - & 99.99 & - \\
& T2 & 99.93 & 91.72 & - & - & - & - & 95.82 & 30.91 \\
& T3 & 99.50 & 94.49 & 99.88 & - & - & - & 97.96 & 64.22 \\
& T4 & 92.24 & 92.68 & 95.89 & 99.99 & - & - & 95.20 & 6.05 \\
& T5 & 92.20 & 92.31 & 95.77 & 97.37 & 98.76 & - & 95.28 & 19.47 \\
& T6 & 99.83 & 89.18 & 97.59 & 97.50 & 81.33 & 99.60 & 94.17 & 41.76 \\

\bottomrule
\end{tabular}

\label{tab:alpha_p1}
\end{table*}

==> ECCV_2026_Paper_Template/sec/0_abstract.tex <==
\begin{abstract}
The rapid advancement of face generation techniques has led to a growing variety of forgery methods. Incremental forgery detection aims to gradually update existing models with new forgery data, yet current sample replay–based methods are limited by low diversity and privacy concerns. Generative replay offers a potential solution by synthesizing past data, but its feasibility for forgery detection remains unclear. In this work, we systematically investigate generative replay and identify two scenarios: when the replay generator closely resembles the new forgery model, generated real samples blur the domain boundary, creating \textbf{domain-risky} samples; when the replay generator differs significantly, generated samples can be safely supervised, forming \textbf{domain-safe} samples. To exploit generative replay effectively, we propose a novel Domain-Aware Relative Weighting (DARW) strategy. DARW directly supervises domain-safe samples while applying a Relative Separation Loss to balance supervision and potential confusion for domain-risky samples. A Domain Confusion Score dynamically adjusts this tradeoff according to sample reliability. Extensive experiments demonstrate that DARW consistently improves incremental learning performance for forgery detection under different generative replay settings and alleviates the adverse impact of domain overlap.
\end{abstract}

==> ECCV_2026_Paper_Template/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
The misuse of deepfake technology is gradually eroding public trust in the online environment, posing serious threats to social security, personal assets, and the political ecosystem. To counter this growing danger, researchers are urgently seeking reliable detection methods to maintain a stable and trustworthy digital media landscape. Current forgery detection methods \cite{sun2022dual,cao2022end,huang2023implicit,yan2024transcending,cheng2024can,cheng2025ed} primarily focus on developing generalized models by fully utilizing existing training samples. However, with the rapid evolution and diversification of forgery techniques, simply improving model generalization is no longer sufficient for real-world applications. Furthermore, when new types of forgeries appear, directly retraining models by combining them with previous samples can lead to excessive computational costs and potential privacy risks. Therefore, developing an effective incremental learning strategy for forgery detection is essential, allowing detection models to continuously adapt and evolve alongside emerging forgery techniques.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figure/intro.pdf}
    \caption{Left: Comparison between traditional sample replay and generative replay. Right: The challenge of applying generative replay to forgery detection, as both Gen-Real and Fake are generated through similar processes, making it difficult for the detector to distinguish real from fake.}
    \label{fig:intro}
\end{figure}

Nowadays, incremental learning–based forgery detection methods typically employ various replay strategies to preserve representative information from previous tasks, including central sample replay \cite{pan2023dfil}, hard sample replay \cite{pan2023dfil}, adversarial perturbations \cite{sun2025continual}, mixed prototypes \cite{tian2024dynamic}, and sparse uniform replay \cite{cheng2025stacking}. These approaches rely on replaying original samples from prior tasks but face two major limitations. We provide a detailed discussion on \textit{\textbf{Related Work}} in Appendix Sec.~\ref{sec:related_work}. As shown in Fig. \ref{fig:intro}, due to limited storage, sample replay can only retain a small subset of representative samples from previous tasks, leading to \textit{\textbf{insufficient data diversity}}. Moreover, storing original forged media introduces \textbf{\textit{privacy and security risks}}. An alternative strategy, generative replay, can effectively address both issues by generating samples instead of storing the originals, thereby avoiding diversity and privacy concerns. However, this approach presents a fundamental challenge for forgery detection, whose goal is to distinguish generated data from real data. The so-called “real” samples produced by generative replay are still synthetic, raising a critical question of whether such data can truly serve as real samples in training forgery detection models.
Motivated by this problem, we make the first attempt to explore the feasibility of generative replay in forgery detection. 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figure/Distribution_illu.pdf}
    \caption{Influence of distribution similarity on generative replay. LDM-I (ODE version~\cite{song2020denoising} of LDM) generates images more similar to LDM than image-level DDPM (using SDE) and DDIM. All replay generators are controlled to have comparable FID scores, ensuring similar generation quality. However, under such a constrained condition, when the replay distribution is closer to the original fake distribution, detection accuracy drops, indicating that generative replay performs better when the replay generator differs more from the deepfake generator.}
    \label{fig:dist-intro}
\end{figure}

As shown in Fig. \ref{fig:dist-intro}, we study generative replay using LDM-generated fake faces together with real faces to train a detection model. Four generators, LDM \cite{rombach2022high}, LDM-I \cite{rombach2022high}, DDIM \cite{song2020denoising}, and DDPM \cite{ho2020denoising}, are used to replay both fake and real distributions, with comparable FID values maintained to ensure fairness. The results show that when the replay generator closely resembles the fake model, such as LDM or LDM-I, the generated samples are poorly distinguished as real or fake. In contrast, generators that differ more from the fake model, such as DDIM or DDPM, achieve accurate detection. These observations suggest that generative replay can be effective in some scenarios but unreliable in others. We refer to the reliable cases as \textbf{domain-safe} and the unreliable ones as \textbf{domain-risky}. Understanding the underlying factors that determine whether a scenario is domain-safe or domain-risky is crucial for designing robust replay strategies.

To fully exploit generative replay for Generated Face Forgery Detection, we propose a Dual \underline{C}onfusion-\underline{A}ware \underline{RE}gularization (Dual-CARE) strategy. The key challenge lies in effectively utilizing replayed samples while mitigating the domain confusion introduced by generative artifacts. To address this, we first introduce a Domain-aware Confusion Score (DC Score) to quantify the degree of domain confusion during training, which is then used to \textbf{dual-modulate} the loss tradeoff in both generator updating and detector learning. Based on this score, we train a pair of updating replay generators that progressively simulate the distributions of all previous-task domains. A domain-aware fast training scheme guided by the DC Score is adopted to enhance the stability and efficiency of generator updating. For detector training, replayed samples are further categorized into “domain-safe” and “domain-risky” groups. The domain-safe samples are directly used for supervised training, while for domain-risky samples we introduce a Relative Separation Loss (RS Loss) to balance the supervision between informative forgery cues and potential confusion introduced by generative artifacts. Extensive experiments demonstrate that Dual-CARE effectively improves detection performance across different replay generators while alleviating the negative effects of domain overlap in incremental deepfake detection. Our contributions can be summarized as follows:
\begin{itemize}
    \item We are the first to explore the feasibility of applying generative replay to generated face forgery detection, analyzing how the overlap between generated “real” and fake samples introduces domain risks that challenge traditional replay assumptions.
    \item We propose Dual-CARE to utilize replayed samples while mitigating interference from generative artifacts, introducing RS Loss and DC Score to adaptively balance information preservation and confusion suppression.
    \item Extensive experiments demonstrate that Dual-CARE consistently enhances incremental detection accuracy across various replay generators and alleviates the negative effects of domain overlap.
\end{itemize}
%-------------------------------------------------------------------------


==> ECCV_2026_Paper_Template/sec/2_related_work.tex <==
\section{Related Works}
\label{sec:related_work}

\subsection{Face Forgery Detection}
Current face forgery detection methods typically leverage available forgery samples to train a generalized model capable of handling unseen forgeries. Various forgery-specific patterns, such as noise \cite{li2020face}, local region \cite{chen2021local,zhao2021multi}, and frequency information \cite{qian2020thinking,guo2020learning,kashiani2025freqdebias}, are explored to capture more discriminative forgery cues. To alleviate the performance degradation observed in cross-domain evaluations, researchers propose a range of learning strategies from different perspectives, including contrastive learning \cite{sun2022dual}, identity information modeling \cite{huang2023implicit,dong2023implicit}, disentangled representation learning \cite{liang2022exploring,yan2023ucf}, reconstruction-based learning \cite{cao2022end,wang2021representative}, and data augmentation \cite{chen2022self,shiohara2022detecting,yan2024transcending}. Recently, several ViT-based methods such as CLIP \cite{cui2025forensics} and LoRA-based Effort \cite{yan2025effort} are proposed to enhance the generalization capability of forgery detection by leveraging large vision-language models. In summary, many general approaches have been proposed to learn transferable forgery features from limited known data. These methods aim to maintain good performance on unseen samples. However, given the large scale and diversity of existing forgery data, relying on a few known datasets to train a truly universal detector is unrealistic.

\subsection{Incremental Learning for Forgery Detection}
Incremental learning has been extensively studied across various domains and is typically categorized into parameter isolation \cite{de2021continual}, parameter regularization \cite{aljundi2018memory,kirkpatrick2017overcoming,li2017learning}, and data replay \cite{mai2021supervised,rebuffi2017icarl}. In the field of face forgery detection, most incremental methods are based on sample replay, where representative samples from previous tasks are stored or reused to mitigate catastrophic forgetting. Representative replay-based approaches in incremental face forgery detection have adopted different strategies to preserve prior knowledge. For example, CoReD \cite{kim2021cored} relies on distillation loss to maintain knowledge from previous tasks. Meanwhile, DFIL \cite{pan2023dfil} improves replay effectiveness by emphasizing both center and hard samples. In addition, HDP \cite{sun2025continual} employs refined universal adversarial perturbations as a replay mechanism. Similarly, DMP \cite{tian2024dynamic} constructs mixed prototypes to summarize earlier task distributions. More recently, SUR-LID \cite{cheng2025stacking} introduces sparse uniform replay combined with a latent-space incremental detector to better preserve previous knowledge. Although effective in retaining previous knowledge, all these methods depend on explicit access to stored samples, which may raise privacy concerns and limit scalability.

Beyond sample-based replay, generative replay offers a promising alternative, reconstructing past distributions through generation rather than storage. This idea has been widely explored in general continual learning, where generative models synthesize pseudo-data to approximate previous task distributions and thus preserve earlier knowledge without explicit memory buffers. The seminal work Deep Generative Replay \cite{shin2017continual} introduces a dual-model framework that reconstructs past data distributions without storing real samples. Building on this idea, data-free class-incremental learning methods \cite{smith2021always} synthesize pseudo-samples through model inversion to enable continual learning under memory and privacy constraints. More recently, diffusion-based generative replay approaches such as DDGR \cite{gao2023ddgr} and SDDGR \cite{kim2024sddgr} have improved the stability and diversity of generated data, achieving stronger knowledge retention in incremental classification and detection tasks. These advances demonstrate the growing potential of generative replay in continual visual learning, though its application to forgery detection remains largely unexplored.


==> ECCV_2026_Paper_Template/sec/3_method.tex <==
\section{Motivation}\label{sec:moti}
As illustrated in Fig. \ref{fig:dist-intro}, when the replay generator differs from the forgery generator, the generation artifacts shared by the replayed real and fake samples remain comparable and therefore do not interfere with the detector’s learning. In contrast, when the replay generator closely resembles the forgery generator, its own generative artifacts are likely to be interpreted as forgery cues. This misalignment causes the replayed real samples to drift away from the true real distribution, thereby confusing the detector. We refer to this phenomenon as the \textbf{Domain Confusion Effect}.

Upon closer examination, this effect indicates that the replayed fake samples themselves do not substantially affect detection performance, regardless of the replay generator used. The core issue instead lies in the replayed real samples, which cannot always be safely used for training. Although their FID suggests that they approximate the original real distribution, these samples still contain subtle synthetic artifacts that can distort the classifier’s decision boundary. Therefore, the key challenge is to leverage the informative content embedded in these replayed real samples while mitigating their generative bias. Moreover, when the replay generator is dissimilar to the original forgery generator, the replayed real samples tend to be less disruptive and can be directly used for classifier training. Consequently, developing a unified learning strategy that remains effective across different replay generators becomes essential for robust generative replay in forgery detection.
\section{Methodology}
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figure/PipelineV4.pdf}
    \caption{Overall framework of our method. We propose a dual confusion-aware regularization strategy to formulate the training of both generation and detection, thereby enabling the integration of generative replay into generative deepfake detection.}
    \label{fig:main-arch}
\end{figure*}
%TODO: 流程图要改； 方法的写作顺序可能要调整(先generation还是先detection) 
\subsection{Overall Framework}
In this paper, we propose a Dual \underline{C}onfusion-\underline{A}ware \underline{RE}gularization (Dual-CARE) Strategy to fully exploit the potential of generative replay for Generated Face Forgery Detection. Specifically, we first introduce the Domain-aware Confusion score (DC Score) to quantify the current condition of the domain confusion issue, thus \textbf{dual-modulating} the loss tradeoff of both generator and detector training. Then, we train a pair of updating replay generators to generate replay data that simulates all previous-task domains, with a domain-aware fast training strategy that leverages DC Score to enhance generative performance. Finally, we deploy the ``domain-safe'' samples to directly supervise the incremental deepfake detector, and we introduce Relative Separation Loss (RS Loss) as a tradeoff with the direct supervision for the ``domain-risky'' samples. The overall framework of our method is shown in Fig.~\ref{fig:main-arch}.

\subsection{Domain-aware Confusion Score}
Here, we firstly design a Domain-aware Confusion Score to quantify the domain confusion issue, i.e., the situation between current generative forgery data and the deployed replay generation model. Given the absence of a clear boundary between domain-risky and domain-safe data, we introduce the Domain-aware Confusion Score (DC Score) to quantify the degree of domain confusion, and dynamically allocate the weights of direct and relative constraints accordingly. Firstly, with a group of images $\mathbf{X}$, we formally define their centroid as:
\begin{equation}
Cent(\mathbf{X}) = \frac{1}{|\mathbf{X}|} \sum_{\mathbf{x} \in \mathbf{X}} f(\mathbf{x}), \label{eq:center}
\end{equation}
where $f(\cdot)$ is the backbone feature extractor. Based on Eq.~\ref{eq:center}, given the generated real samples from all past tasks $\mathcal{D}^{r\text{-gen}}_t$ and the current task's fake data $\mathcal{D}_{t+1}^{f}$, we can obtain their centroids as $Cent(\mathcal{D}^{r\text{-gen}}_t)$ and $Cent(\mathcal{D}_{t+1}^{f})$. Then, we employ L2 distance to quantify the overall \textbf{distance} between them as: \begin{equation}     
    s_{t+1}= \|Cent(\mathcal{D}^{r\text{-gen}}_t) - Cent(\mathcal{D}_{t+1}^{f})\|_2. 
    \label{eq:dcs_dist} 
\end{equation} 
We adopt $s_{t+1}$ with different normalizations as the DC score since it provides a direct measure of distribution separation, where a smaller distance indicates a higher risk of confusion.

\subsection{Diffusion Replay Generation for Deepfake Detection}

\paragraph{\textbf{General Training Pipeline of Diffusion Generator.}}
Given a set of Deepfake detection training data as $\mathcal{D}=\{\mathcal{D}^{f},\mathcal{D}^{r}\}$, we deploy Latent Diffusion Model (LDM) as our generator backbone considering the superior performance of the advanced diffusion model. Then, since $\mathcal{D}^{fake}$ and $\mathcal{D}^{real}$ contain opposite information for detector training, two generators are assigned to each real/fake domain to learn their information, respectively. Learning one domain for the generator could be written as:
\begin{equation}
\mathcal{L}_{G^{(\cdot)}}(\mathcal{D}^{(\cdot)}) = 
\mathbb{E}
\left[
\left\| 
\epsilon - \epsilon_{\theta}\left(\mathbf{x}_s,\, s,\, \mathbf{c}\right)
\right\|_2^2
\right], \label{eq:gen}
\end{equation}
where ${\mathbf{x}\sim \mathcal{D}^{(\cdot)},\, \epsilon\sim\mathcal{N}(0,1),\, s\sim \mathcal{U}(1,S)}$. Based on Eq.~\ref{eq:gen}, we can obtain a pair of trained generators $\mathbf{G}=\{G^f,G^r\}$. 

\paragraph{\textbf{Generative Replay for All Previous Tasks in Deepfake Detection.}}
Here, we aim at obtaining replay samples $\mathbf{R}^{\text{gen}}_t$ for $(t+1)$-task incremental learning via diffusion generative replay. To reduce the memory overhead incurred by generative replay to O(1), we employ two generators $\mathbf{G}_t = \{ G_t^f, G_t^r \}$ to replay all real and fake data from $t$-th task and before, rather than learning the $t$-th task in isolation and allocating independent generators for each previous task.

Specifically, following DDGR~\cite{gao2023ddgr}, we leverage the generator $\mathbf{G}$ trained on the ($t-1$)-th task to synthesize a replay dataset $\mathcal{D}_{t-1}^{\text{gen}}$, which can iteratively represent all task that $\leq (t-1)$. This generated dataset is subsequently combined with the current task dataset $\mathcal{D}_t$ for joint training. Formally, the training data $\mathcal{\hat{D}}_t$ for $\mathbf{G}_{t}$ can be written as:
\begin{equation}
    \mathcal{\hat{D}}_t=\{\mathcal{D}_t^{(\cdot)},\mathcal{D}_{t-1}^{(\cdot)\text{-gen}}\},
\end{equation}
where $(\cdot)$ could be either real ($r$) or fake ($f$). In this manner, the updated generator $\mathbf{G}_t$ is encouraged not only to acquire knowledge from the new task but also to preserve its generative capability on previously learned tasks. 
\paragraph{\textbf{Domain-aware Fast Training.}}
Then, considering that the generator’s performance in simulating different data distributions is intrinsically correlated with the characteristics of the distributions themselves, we introduce the confusion coefficient to regularize the learning process of the generator. Specifically, we first decouple the training gradients induced by the previous and current data, which yields:
%Then, 考虑到生成器的在模拟不同分布时的表现与分布本身的特质密切相关，我们引入了混淆系数来regularize生成器的学习过程。具体的说，我们首先将previous 和 current数据的训练梯度解耦开来，可以得到:
$\mathcal{L}_{G^{(\cdot)}}(\mathcal{\hat{D}}_t^{(\cdot)})=\mathcal{L}_{G^{(\cdot)}}(\mathcal{D}_t^{(\cdot)})+\mathcal{L}_{G^{(\cdot)}}(\mathcal{D}_{t-1}^{(\cdot)\text{-gen}})$.
For the real generator $G^{r}$, our objective is to approximate multiple real domains as faithfully as possible. The real domains and the synthetic artifacts introduced by the generator itself are not inherently conflicting during the generation process. The potential conflict with fake domains arises primarily during detection, which should therefore be addressed through appropriate design at the detector training stage. Consequently, $G^{r}$ is expected to be effective in the acquisition of new knowledge while preserving previously learned knowledge. Hence, no additional weighting mechanism is required for $G^{r}$. 

However, the fake generator $G^{f}$ necessitates additional design considerations. This is because the generated fake samples inherently contain the generator’s intrinsic fabrication patterns, rendering their relationship with newly learned forgery characteristics substantially more intricate. To facilitate more stable training and improved performance of the fake generator, we hence introduce the confusion coefficient to adaptively balance the training weights, which can be formulated as:
\begin{equation}
  \mathcal{L}_{G^{f}}(\mathcal{\hat{D}}_t^{f})=(1-s_{t})\times\mathcal{L}_{G^{f}}(\mathcal{D}_t^{f})+s_{t}\times\mathcal{L}_{G^{f}}(\mathcal{D}_{t-1}^{f\text{-gen}}).  
\end{equation}
As $s_t$ increases, the discrepancy between the current-task forgery artifacts and the generator-inherent characters becomes more pronounced. In such cases, the gradient conflict introduced by new information intensifies, and it becomes more crucial to preserve previously acquired knowledge to prevent it from being completely overridden. Accordingly, the weight assigned to prior information should be increased, enabling gradual adaptation, safeguarding performance, and promoting convergence toward a more favorable local optimum.
Conversely, when $s_t$ is small, the gap between the current task and the generator is limited, and the conflict induced by new knowledge is correspondingly mild. Under this condition, a larger learning weight can be assigned to the new information gradient, which facilitates faster convergence while maintaining stability.

%对于real 生成器，我们的目标就是尽可能的拟合多种real domain，real domain 与gen自身的伪造信息，在生成时并不冲突。而在检测时与fake domain冲突的问题，我们应该在检测器的训练端进行相关设计。因此，real_gen只需要正常的做到学习新知识且保留旧知识即可，这就是最有利的情况。所以，对于real 生成器我们并不需要额外的增加权重
%而fake 生成器则需要进行额外的设计: 因为fake的生成信息中，包含了生成器自带的伪造信息，这与所学的伪造的关系更加复杂。为了更好的帮助fake_gen的训练和表现，我们考虑利用混淆系数自适应的平衡data_p_gen和data_cur的训练权重，which can be written as:. 显然，n越大，当前任务和生成器的差距越大，此时新信息冲突更大，因此更要尽可能保护过往信息，防止被新的信息给完全覆盖了，所以得提高过往信息权重，慢慢学习，保护性能，探索更好的局部最优解。而n越小，差距越小，需要学的东西也冲突更小，因此可以更大的学习新信息，有利于快速收敛。


%为了将引入生成回放的存储消耗降低至O(1)，我们考虑使用两个生成器$\mathbf{G}_t=\{G^f_t,G^r_t\}$来回放(t)-task的所有real/fake data，而不是仅仅学习t-task，然后为每一个task均分配各自的生成器. To achieve that, following DGR, 我们考虑利用在 (t-1)-task上所学的$\mathbf{G}_{t-1}$生成一组$\mathcal{D}_{t-1}^{gen}$，然后将其与t任务的$\mathcal{D}_t$混合同时进行训练。这样，我们就能约束$\mathbf{G}_t$既学到新任务的知识，又能维持老任务的生成性能。
\paragraph{\textbf{Final Summarized Samples for Detector Training.}}
During incremental learning of deepfake detectors,  $\mathbf{G}$ will provide the generative replays $\mathbf{R}^{\text{gen}}_t=\{\mathcal{D}_{t}^{f\text{-gen}},\mathcal{D}_{t}^{r\text{-gen}}\}$, which will be combined with the next ($t+1$)-th data for training. During ($t+1$)-th task, the training mini-batch is the combination of generative real/fake replay and ($t+1$)-th data, which can be written as $\mathbf{X}_{t+1}=\{\mathbf{X}^r_{t+1},\mathbf{X}^f_{t+1},\mathbf{X}_g^r,\mathbf{X}_g^f\}$, where each $\mathbf{X}^{(\cdot)}_{(\cdot)}$ is a group of corresponding $\mathbf{x}^{(\cdot)}_{(\cdot)}$, while $\{\mathbf{X}^r_{t+1},\mathbf{X}^f_{t+1}\}\subseteq\mathcal{D}_{t+1}$ and $\{\mathbf{X}_g^r,\mathbf{X}_g^f\} \subseteq \mathbf{R}^{\text{gen}}_t$.


\subsection{Training Deepfake Detector with Generative Replay}
\paragraph{\textbf{Relative Separation Loss.}}
As previously discussed, domain confusion among generative real replays, actual real samples, and actual fake samples may mislead the detector when direct label-based supervision is conducted. However, the similar learning effectiveness between domain-safe\&real and domain-risky\&real suggests that the domain-risky samples also contain previous information that could be beneficial to mitigating the catastrophic forgetting. Therefore, we propose the Relative Separation Loss (RS Loss) to leverage the valuable previous information. Instead of explicit real-fake supervisions, RS Loss considers from an indirect relative perspective. Specifically, despite the domain-risky $\mathbf{x}_g^r$ may exhibit similarity with current fake samples, its relative relation with $\mathbf{x}_g^f$ should be consistent. This is because both $\mathbf{x}_g^r$ and $\mathbf{x}_g^f$ are generated by the same real domain and the same generative character. As a result, the distinction between them is effectively nullified and filtered, leaving only the $t$-th forgery character. Consequently, the distribution of $\mathbf{x}_g^f$ and $\mathbf{x}_g^r$ could be encouraged to separate if they correspond to domain-risky samples. 
% To be specific, given a minibatch $\mathbf{X}$, we firstly calculate the feature centroids of $\mathbf{X}^r_g$ and $\mathbf{X}^f_g$ as:
% \begin{equation}
%     Cent(\mathbf{X}^r_{(\cdot)}) = \frac{1}{n} \sum_{k=1}^{n} f(\mathbf{X}^r_{(\cdot)}), \label{eq:center}
% \end{equation}
% where $f(\cdot)$ is the backbone feature extractor. Then, we define RS Loss as enlarging the distance between $Cent(\mathbf{X}^f_\text{gen})$ and $Cent(\mathbf{X}^f_\text{t+1})$, which could be written as:
% \begin{equation}
%     L_\text{rs}=-||Cent(\mathbf{X}^f_\text{gen})-Cent(\mathbf{X}^f_\text{t+1})||_2.
% \end{equation}

To be specific, given a minibatch $\mathbf{X}$, we first calculate the feature centroid of the generated real samples $\mathbf{X}^r_g$ based on Eq.~\ref{eq:center}, denoted as $Cent(\mathbf{X}^r_g)$.
% \begin{equation}
% Cent(\mathbf{X}^r_g) = \frac{1}{|\mathbf{X}^r_g|} \sum_{\mathbf{x} \in \mathbf{X}^r_g} f(\mathbf{x}), \label{eq:center}
% \end{equation}
Then, we define RS Loss to maximize the separation between this generated real centroid and each sample-wise generated fake feature $\mathbf{x} \in \mathbf{X}^f_g$. This is achieved by minimizing their average cosine similarity, which can be written as:
\begin{equation}
\mathcal{L}_\text{rs} = \frac{1}{|\mathbf{X}^f_g|} \sum_{\mathbf{x} \in \mathbf{X}^f_g} \frac{f(\mathbf{x}) \cdot Cent(\mathbf{X}^r_g)}{\|f(\mathbf{x})\|_2 \cdot \|Cent(\mathbf{X}^r_g)\|_2}. \label{eq:rs_loss}
\end{equation}
RS Loss can leverage the previous information in the replay real sample by sample. By considering the relative authenticity differences among generated images, we indirectly exploit the information embedded within the generative replay, even when they are domain risky.
 %通过利用gen image的相对真伪差异，我们以间接的方式利用了Gen里包含的信息，哪怕这些数据是domain risky的。
% Firstly, given $\mathbf{R}_g^f$ and $\mathcal{D}^{real}_{t+1}$, we also obtain their centroids based on Eq.~\ref{eq:center} as $Cent({f}(\mathbf{R}_g^f))$ and $Cent(f(\mathcal{D}^{real}_{t+1}))$.Then, we employ Cosine Similarity to quantify the overall similarity between the two distributions as:
% \begin{equation}
%     s_{t+1}=\frac{Cent(f(\mathbf{R}_g^f)) \cdot Cent(f(\mathcal{D}^{real}_{t+1}))}
% {\left\|Cent(f(\mathbf{R}_g^f))\right\| \, \left\|Cent(f(\mathcal{D}^{real}_{t+1}))\right\|}.
%  \end{equation}
% We adopt cosine similarity as it quantifies the similarity in directional vectors, thereby eliminating potential interference arising from real-domain similarities.
\paragraph{\textbf{Overall Detection Loss.}}
When domain confusion is relatively mild, direct supervision evidently provides strong guidance. Meanwhile, RS Loss facilitates maximal exploitation of the informative content within domain-risky data. Therefore, we propose to adaptively adjust the balance between RS Loss and direct supervision. 
Hence, by incorporating RS Loss and DC Score, we formulate a unified loss function that simultaneously optimizes both domain-risky and domain-safe samples for generative replay-based deepfake detection.
Firstly, the common supervision signal for face forgery detection is a Cross-Entropy loss, which could be written as:
\begin{equation}
        \mathcal{L}_{\text{ce}}(\mathbf{x}) = - \left( \hat{y} \log(y_p) + (1 - \hat{y}) \log(1 - y_p) \right),\label{eq:celoss}
\end{equation}
where $\hat{y}$ is the corresponded ground-truth label, $y$ is the predicted result from the backbone. Since $\forall\,\mathbf{x} \in \left\{ \mathbf{X}^r_{t+1},\ \mathbf{X}^f_{t+1},\ \mathbf{X}_g^f \right\}$ $\mathbf{x}$ is \textit{confusion-free} based on the discussion in Sec.~\ref{sec:moti}, we can directly constrained them by $\mathcal{L}_\text{cf}=\mathcal{L}_{ce}(\mathbf{x})$. Then, we separate $\tilde{\mathbf{x}} \in \mathbf{X}_g^r$ from $\mathbf{X}$ that could \textit{confuse} to adaptively adjust the direct and relative constraints based on DC Score, which can be written as:
\begin{equation}
     \mathcal{L}_{\text{c}}=s_{t+1} \mathcal{L}_{ce}(\tilde{\mathbf{x}})+ (1-s_{t+1}) \mathcal{L}_{rs},
\end{equation}
which means the safe direct supervision could be conducted with higher weights if the domain distance is relatively large, otherwise a higher $L_{rs}$ should be applied.
% \begin{equation}
%     L_{\text{risky}}=(1-\alpha_{t+1}) L_{ce}(\tilde{\mathbf{x}})+ \alpha_{t+1} L_{rs}.
% \end{equation}

Therefore, the overall loss can be written as:
\begin{equation}
    \mathcal{L}_{overall}=\mathcal{L}_\text{c}+\mathcal{L}_\text{cf},
\end{equation}
which encourages the detector to leverage information from current and replay samples simultaneously.
% $G(\cdot,\theta_g)$, where $\theta_g$ is the trainable parameter

%to measure the domain similarity 

==> ECCV_2026_Paper_Template/sec/4_experimental.tex <==
\section{Experimental Results}

\subsection{Experimental Settings}

\subsubsection{Datasets.}
To construct a comprehensive and challenging benchmark for incremental face forgery detection, our experiments utilize a curated selection of datasets, which is designed to simulate a realistic scenario by spanning both classical, widely-used forgery datasets and the latest cutting-edge forgeries generated by advanced diffusion models. The classical datasets include: Celeb-DF-v2 (CDF)~\cite{Celeb-df}, DeepFake Detection Challenge Preview (DFDCP)~\cite{dfdc}, and the hybrid-category FaceForensics++ (FF++)~\cite{FF++}. To address the most recent threats, we further incorporate a suite of modern forgeries, that is, \{SDv21~\cite{sdv15}, DiT~\cite{DiT}\} from DF40~\cite{df40} and \{LDM~\cite{rombach2022high}, DDPM~\cite{ho2020denoising}\} from DiffusionFace~\cite{diffusionface}. This blend of classical and cutting-edge forgery types creates a comprehensive evaluation against evolving threats.

% 数据集。 为了构建一个全面且富有挑战性的增量式人脸伪造检测基准，我们的实验采用了一组精心挑选的数据集。这一选择旨在模拟一个真实的场景，它既涵盖了经典的、被广泛使用的伪造数据集，也包括了由先进的扩散模型生成的最新前沿伪造。经典数据集包括已建立的基准，如 Celeb-DF-v2 (CDF)、DeepFake Detection Challenge Preview (DFDCP)，以及混合类别的 FaceForensics++ (FF++)。为了应对最新的威胁，我们进一步纳入了一套现代伪造数据集，即来自 DF40 的 {SDv21, DiT} 和来自 DiffusionFace 的 {LDM, DDPM}。这种“经典”与“前沿”伪造类型的混合，为评估模型应对不断演变威胁的鲁棒性创造了一个高度真实的测试平台。

\subsubsection{Incremental Protocols.}
To comprehensively evaluate model robustness in evolving forgery landscapes, we propose two complementary incremental protocols that capture real-world dynamics and benchmark-level comparability.

 % 为了全面评估模型在不断演化的人脸伪造场景中的鲁棒性，我们提出了两种互为补充的增量协议，以同时捕捉真实世界动态与基准级可比性。

\begin{itemize}

\item \textbf{Protocol 1 (P1): Mixed-Era Forgery Incremental.}
It follows the sequence \{LDM, DFDCP, SDv21, DDPM, DiT, CDF\}, simulating a realistic, temporally chaotic evolution of forgery techniques. It intentionally interleaves classical Face-Swapping (FS) datasets (DFDCP, CDF) with modern Entire Face Synthesis (EFS) forgeries to emulate the heterogeneous and non-sequential emergence of threats in the wild. This setup is designed to rigorously evaluate the resilience of a model to catastrophic forgetting and its adaptability to domain confusion.

 % 该协议采用数据序列 {LDM, DFDCP, SDv21, DDPM, DiT, CDF}，旨在模拟一个真实且时间上混乱的伪造技术演化过程。序列中有意交织了经典的人脸替换（Face-Swapping, FS）数据集（DFDCP、CDF）与现代的整脸合成（Entire Face Synthesis, EFS）伪造数据，以仿真真实环境中威胁的异质性与非顺序性出现模式。此设置旨在严格测试模型在面对突发的数据分布变化时的抗灾难性遗忘能力与自适应能力。

\item \textbf{Protocol 2 (P2): Benchmark-Aligned Incremental.}  
It employs the sequence \{DDPM, FF++, DFDCP, CDF\} and extends the benchmark protocol introduced in recent work SUR-LID. To maintain alignment with prior baselines while avoiding redundant configurations, we replace the initial dataset (SDv21) with DDPM, a diffusion-based forgery type. This modification ensures consistency with established benchmarks while incorporating emerging generative paradigms for a fair yet forward-looking evaluation.

\end{itemize}

 % 该协议采用数据序列 {DDPM, FF++, DFDCP, CDF}，并在近期文献 SUR-LID 提出的基准协议基础上进行了扩展。为在保持与已有基线一致的同时避免冗余配置，我们将原协议的初始数据集（SDv21）替换为另一种基于扩散模型的伪造类型 DDPM。此修改确保了与既有基准的一致性，同时引入了新兴生成范式，从而实现公平且具前瞻性的评估。

\subsubsection{Implementation Details.}
Our framework is built upon the EfficientNetB4~\cite{effnet} backbone. We train all models using the Adam optimizer~\cite{adam} with a learning rate of 0.0002 for 5 epochs. All inputs are resized to 256$\times$256 and processed with a batch size of 32. For baseline methods that rely on replaying original samples, we set the replay buffer size to 500 samples per task. To ensure a fair and reproducible comparison, all baseline methods were carefully replicated within the standardized DeepFakeBench~\cite{deepfakebench}. We report Frame-level Area Under Curve (AUC)~\cite{deepfakebench} as the primary evaluation metric, supplemented by accuracy (ACC) for comprehensive alignment with existing methods. Furthermore, we define a Performance Dropping rate (PD) to quantify the absolute performance drop for catastrophic forgetting, calculated as $PD = M_0 - M_N$, where $M_0$ is the average metric (AUC or ACC) in the base session and $M_N$ is the average metric in the final session. All experiments were performed on a NVIDIA Tesla A100 GPU.

% 实现细节。我们的检测框架基于 EfficientNetB4 骨干网络构建。我们使用 Adam 优化器训练所有模型，学习率为 0.0002，共训练 5 个 epoch。所有输入图像均被调整为 256$\times$256，并以 32 的批处理大小进行处理。对于那些依赖回放真实样本的基线方法，我们将每个任务的重放缓冲区大小设置为 500。为确保公平且可复现的比较，所有基线方法均在标准化的 DeepFakeBench 平台内被仔细复现，并且包括预处理在内的所有实验都严格遵守其官方 settings。我们报告帧级曲线下面积 (AUC) 作为主要评估指标，并辅以准确率 (ACC) 以便与现有方法进行全面对齐。此外，我们定义了一个性能下降率 (PD) 来量化绝对的性能下降 ，计算公式为 $PD = M_0 - M_N$，其中 $M_0$ 是模型在基础会话（base session）中的平均指标（AUC或ACC），而 $M_N$ 是其在最终会话中的平均指标 。 所有实验均在 一台 NVIDIA GeForce RTX 3080 GPU 上执行。

\input{tab/p1}

\subsection{Comparisons with Existing Methods}
We compare our method against key baselines on Protocol 1, including general continual learning methods (LwF~\cite{li2017learning}, iCaRL~\cite{rebuffi2017icarl}, DER~\cite{yan2021dynamically}) and state-of-the-art IFFD-specific methods (CoReD~\cite{kim2021cored}, HDP~\cite{sun2025continual}, DFIL~\cite{pan2023dfil}, SUR-LID~\cite{cheng2025stacking}).
As shown in Tab.~\ref{tab:main_comparison}, our method consistently outperforms all baselines under Protocol 1 and achieves the highest average AUC across incremental tasks, while requiring \textbf{no} actual data replay. This advantage mainly arises from two aspects. First, generative replay is able to approximate the data distributions of previous tasks and produce diverse rehearsal samples, which helps the model preserve historical knowledge without storing real images. Second, the proposed confusion-aware regularization enables the model to exploit replay samples more effectively by distinguishing between reliable and ambiguous supervision signals. As a result, related forgery tasks can facilitate knowledge transfer while reducing negative interference, leading to improved stability and stronger incremental learning ability. Please refer to the \textit{Appendix} for comparisons on Protocol 2.

\subsection{Ablation Study}
Here, we validate the component performance of the proposed Dual-CARE. As shown in Tab.~\ref{tab:ablation}, we first demonstrate the effectiveness of DC-guided generation. The training curves in Fig.~\ref{fig:loss} further validate that our domain-aware strategy effectively facilitates faster convergence when $s_t$ is small, perfectly aligning with our theoretical design.

Then, in order to concisely investigate the effectiveness of the detector training strategy, we have isolated the components of the detector training process by setting all remaining ablation variables without any generator strategy, considering that the training strategy of the detector is the core solution to domain confusion. 
It can be observed that removing Gen-Real supervision causes a substantial performance drop, underscoring the importance of explicit label guidance for generated samples. Similarly, omitting $\mathcal{L}_{rs}$ reduces performance significantly. The reluts confirm that direct supervision and relative separation are complementary and both crucial for mitigating generative artifacts and maintaining accurate decision boundaries. Moreover, we analyze the impact of distance metrics used in DC Score and $\mathcal{L}_{rs}$. All metric combinations outperform the variants without $\mathcal{L}_{rs}$, while DCS-L2 + RS-Cos achieves the best performance. This suggests that using L2 for the DCS  better captures domain confusion, while cosine similarity is more effective in enforcing feature separation in $\mathcal{L}_{rs}$. 

Furthermore, we also specifically conduct a series of supplementary analyses, covering different backbone choices, alternative normalization functions for computing the adaptive weight $\alpha$, as well as sample-wise versus centroid-based variants of $\mathcal{L}_{rs}$. Please refer to the \textit{Appendix} for details.

\input{tab/ablation}

% 我们验证了核心组件的有效性：Gen-Real 直接监督 (Eq. 7) 和相对分离损失 ($\mathcal{L}_{rs}$) (Eq. 3)，以及对 DCS 和 $\mathcal{L}_{rs}$ 的距离度量（L2 与 Cosine）的敏感性。结果汇总于表 \ref{tab:ablation}。


% 组件消融。 如表 \ref{tab:ablation} 所示，移除 Gen-Real 监督导致性能显著下降（平均AUC 0.7432），凸显了对生成样本进行显式标签引导的必要性。此外，移除 $\mathcal{L}_{rs}$ 也会将性能降低至 0.9097。这证实了直接监督和相对分离是互补的，对于减轻生成伪影和维持准确的决策边界至关重要。

% 距离度量分析。 关于距离度量，虽然所有组合都优于消融后的变体，但 DCS-L2 + RS-Cos 配置取得了最佳性能（平均 AUC 0.9498）。这表明 L2 距离能更好地衡量域冲突 (DCS)，而余弦相似度则更有效地用于特征分离 ($\mathcal{L}_{rs}$)。



% 如表 \ref{tab:Generation analysis} 所示，结果清晰地展示了非自适应策略的缺陷。“仅伪造回放”策略遭受了严重的性能下降，在 T6 的最终平均AUC仅为 0.7856，这表明完全丢弃 Gen-Real 样本会导致灾难性的遗忘。相反，“全回放”策略的表现要好得多 (平均AUC 0.9155)。值得注意的是，两个固定 alpha 的基线（$\alpha=0.5$ 时为 0.9372，$\alpha=0.1$ 时为 0.9312）均优于“全回放”，这表明即使没有动态加权，加入我们的推送损失 ($\mathcal{L}_{rs}$) 也是有益的。我们的动态 Dual-CARE 取得了最佳的整体性能，获得了最高的最终平均AUC (0.9574) 和最低的性能下降率 (PD $\downarrow$ 为 0.0425)。这证实了我们的动态自适应机制能有效平衡知识保留和风险规避，且优于所有固定策略。

\subsection{Analysis of Generative Replay}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{visualization/merged_00.png} 
    \caption{Analysis of generative replay strategy. (Left) Performance vs. replay sample size on P1 and P2. (Right) Impact of replay generator quality (avg. AUC on T2-T4).}
    \label{fig:replay_analysis}
\end{figure}
\begin{figure}[h]
\centering
\begin{minipage}{0.60\textwidth}
  \centering
  \includegraphics[width=\linewidth]{visualization/t2_eta1_dual_11.png}
  \caption{UMAP visualizations. (Left) Initial state: Gen-Real (pink) is ambiguously positioned near Fake (red/cyan). (Right) After learning T2: Our method ($\mathcal{L}_{rs}$) actively separates the Gen-Real cluster, resolving the domain confusion.}\label{fig:feature}
\end{minipage}
\hfill
\begin{minipage}{0.37\textwidth}
  \centering
  \includegraphics[width=\linewidth]{ECCV_2026_Paper_Template/visualization/vloss.pdf}
  \caption{Learning rate with (Ours) or without (Base) Domain-aware Fast Training.}\label{fig:loss}
\end{minipage}
\end{figure}
\begin{figure}[b]
\vspace{-0.3cm}
    \centering
    \includegraphics[width=1\linewidth]{ECCV_2026_Paper_Template/visualization/pic_pri.pdf}
    \caption{Quantitative analysis on privacy protection effectiveness of our method.} 
    % We compute the cosine similarity between the ID embeddings of generated replay samples and the actual training faces across a fully connected cross-comparison matrix ($10,000 \times 10,000$). The FID score demonstrates the overall distributional consistency between generative and actual data, while the similarity results show that each generated faces are very different from any face in the actual dataset, thus indicating a lesser Privacy risk when deploying the generative replay. }
    \label{fig:id-leak}
\end{figure}
\subsubsection{Free Lunch for Replay Diversity.}
Replay diversity is a free lunch for generative replay since it can generate infinite images with a single generator. In contrast, common replay requires equivalent storage burden to achieve an equivalent larger replay size. Here, we showcase the influence of replay diversity to incremental learning and also the achieved diversity of generative replay. In Fig.~\ref{fig:replay_analysis}, it can be observed that increasing the replay size of DFIL can effectively improve its performance, indicating the significance of replay diversity. Similarly, our performance is also enhanced as the generative replay size increase, which demonstrate its improved generative diversity. 
% which could be achieved with \textit{no pain}. (left) plots the final average AUC on both P1 (T6) and P2 (T4) as the sample size increases from 50 to 4000. DFIL's performance is highly dependent on the buffer size, showing a clear trade-off between accuracy and storage cost. In contrast, our generative method (Dual-CARE) achieves superior performance across all data points on both protocols (e.g., 0.9574 on P1 at 4000 samples). Our approach provides diverse samples on-the-fly, achieving superior scalability and practical utility without the linear storage penalty.

% 回放可扩展性。 我们首先分析了回放样本大小相对于基于存储的 DFIL 的影响。图 \ref{fig:replay_analysis} (左) 绘制了在 P1 (T6) 和 P2 (T4) 上，当样本量从 50 增加到 4000 时的最终平均 AUC。DFIL 的性能高度依赖于缓冲区大小，显示了准确性与存储成本之间的明显权衡。相比之下，我们的生成式方法 (Dual-CARE) 在两个协议的所有数据点上均取得了更优越的性能（例如，在 P1 的 4000 样本上达到 0.9574）。我们的方法可以即时 (on-the-fly) 提供多样化的样本，在没有线性存储惩罚的情况下，实现了卓越的可扩展性和实用价值。

\subsubsection{Impact of Generator Quality.}
We further evaluate the impact of the quality of the replay generator on detection performance. As shown in Fig.~\ref{fig:replay_analysis} (right), we compare three different generators (\textit{i.e.}, GAN, DDIM, and LDM) on the P2 protocol. The results show a clear correlation between generation fidelity and detection accuracy. The GAN-based generator exhibits poor performance
due to its simple architecture and outdated mechanism.  LDM and DDIM, as the latest Diffusion-based detectors, can both perform promisingly to generate replays that enhance incremental learning. Hence, we choose to deploy LDM as the generator of our method. Moreover, the similar performance with LDM and DDIM demonstrates that Dual-CARE is not dependent to specific generators unless it being incapable, which indicates its scalability and application potential.

% 生成器质量。 我们进一步评估了回放生成器质量对检测性能的影响。如图 \ref{fig:replay_analysis} (右) 所示，我们在 P2 协议上比较了三种不同的生成器（GAN, DDIM, LDM）。结果显示，生成保真度与检测准确率之间存在明显的相关性。LDM 产生了最高质量的样本，取得了最佳性能，显著优于 DDIM，而传统的 GAN 表现不佳。这表明我们的 Dual-CARE 框架的有效性随着生成模型的进步而提升，凸显了其未来的潜力。

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=1\linewidth]{visualization/t2_eta1_dual_11.png}
%     \caption{UMAP visualization of T1 (LDM) features. (Left) Initial state: Gen-Real (pink) is ambiguously positioned near Fake (red/cyan). (Right) After learning T2: Our method ($\mathcal{L}_{rs}$) actively separates the Gen-Real cluster, resolving the domain confusion.}
    
%     % 表5：T1 (LDM) 特征的 UMAP 可视化。(左) 初始状态：Gen-Real (粉色) 模糊地位于 Fake (红色/青色) 附近。(右) 学习 T2 后：我们的方法 ($\mathcal{L}_{rs}$) 主动将 Gen-Real 簇分离，解决了域混淆问题。
    
%     \label{fig:feature}
% \end{figure}
\subsection{Visualization Analysis on Domain Confusion}

To intuitively analyze the observed domain confusion, we visualize the T1 LDM feature space using UMAP~\cite{umap}. As shown in Fig.~\ref{fig:feature}, the initial Gen-Real samples occupy an ambiguous region, lying close to the Fake clusters and thus presenting a high risk of domain confusion. In contrast, the right plot shows the feature space after incrementally learning T2 DFDCP. Guided by our adaptive mechanism driven by $\mathcal{L}_{rs}$, the ambiguity is effectively resolved: the Gen-Real features are pushed away from the Fake clusters and aligned with the Real cluster. This visualization shows that our method reliably rectifies distributional misalignment and restores clear feature separation.
Additional visualizations across multiple datasets are provided in the \textit{Appendix} to further support these observations. 

% 为了直观地展示我们的自适应机制，我们使用 UMAP 可视化了 T1 (LDM) 的特征空间 (图 \ref{fig:feature})。如 (左图) 所示，初始的 Gen-Real (粉色) 样本占据了一个模糊的位置，靠近 Fake (红色/青色) 簇，带来了很高的域混淆风险。相反，(右图) 显示了增量学习 T2 (DFDCP) 后的特征。我们的自适应机制在 $\mathcal{L}_{rs}$ 的驱动下，成功地解决了这种模糊性：Gen-Real 特征被主动推离 Fake 簇，并与 Real (蓝色) 簇对齐。此可视化证实了我们的方法能有效识别并纠正分布的模糊性。
\subsection{Analysis of Domain Confusion Effect}

\input{tab/Generation_analysis}

To comprehensively analyze the effect of domain confusion, we compare our dynamic generative replay strategy with several key baselines on Protocol 1, with quantitative results presented in Tab.~\ref{tab:Generation analysis}. We evaluate our proposed Dual-CARE against Full Replay, which replays both Gen-Real and Gen-Fake samples, Fake-Only Replay, which discards all Gen-Real samples to entirely prevent the domain confusion effect. We also introduce two fixed-$s_t$ baselines that combine losses with $s_t$ fixed at 0.1 and 0.5. 
% 在本节中，我们通过在协议1 (P1) 上将我们的动态生成式回放策略与几个关键基线进行比较，来分析其功效。量化结果如表 \ref{tab:Generation analysis} 所示。我们评估了我们的方法 Dual-CARE，并将其与“全回放”（同时回放 Gen-Real 和 Gen-Fake 样本）、“仅伪造回放”（丢弃所有 Gen-Real 样本）以及两个固定 alpha 的基线（使用我们方法的损失函数，但将 $\alpha$ 固定为 0.1 和 0.5）进行对比，以分离出我们动态调整机制的影响。
The results show the clear drawbacks of non-adaptive strategies. Fake-Only Replay suffers a severe performance degradation since it completely discards all Gen-Real samples, thus leading to severe catastrophic forgetting. Conversely, Full Replay performs better but falls quickly when domain confusion is encountered. Subsequently, although different strategies that combine loss with fixed value exhibit improved effectiveness, they are still outperformed by our Dual-CARE, which demonstrates that the proposed adaptation strategy effectively balances knowledge preservation and risk mitigation.

\subsection{Privacy Quantitative Analysis}
Traditional sample replay poses privacy risks by storing raw facial images. Generative replay avoids this but may risk identity memorization. To evaluate this, we measure feature similarity between synthesized replay samples and original training faces using ArcFace \cite{deng2018arcface} and CosFace \cite{wang2018cosface}. As shown in Fig.~\ref{fig:id-leak}, similarities are near zero with minimal variance. Despite a high generation fidelity (FID 15.36), the generator produces entirely novel identities by capturing the structural distribution rather than memorizing training samples. This confirms that our generative replay framework effectively mitigates identity leakage, providing a secure rehearsal mechanism for incremental deepfake detection.
% \begin{table}[t]
%     \centering
%     \small\setlength{\tabcolsep}{5pt}
%     \caption{Quantitative Analysis of GenReplay Privacy and Generation Quality. The Global Mean and Variance represent the cosine similarity between the generated replay samples and the actual training faces across a fully connected cross-comparison matrix ($10,000 \times 10,000$). The FID score evaluates the overall data distribution fidelity.}
%     % 身份隐私的定量分析。全局均值和方差代表了在全连接交叉比对矩阵中，生成的回放样本与实际训练人脸之间的余弦相似度。FID得分评估了整体数据分布的保真度。
%     \begin{tabular}{c|ccccc}
%         \toprule
%         \textbf{Method} & \textbf{Arc Mean} & \textbf{Arc Var} & \textbf{Cos Mean} & \textbf{Cos Var} & \textbf{FID $\downarrow$} \\
%         \midrule
%         \textbf{GenReplay (Ours)} & 0.0177 & 0.0048 & 0.0172 & 0.0047 & 15.36 \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:privacy_gen}
% \end{table}



% 传统样本回放的一个主要局限在于存档原始人脸图像所固有的隐私风险。生成式回放通过合成历史数据自然地规避了这一存储限制；然而，它引入了身份记忆的潜在风险，即生成器可能会无意中重建特定的训练人脸。为了严格评估这一隐私担忧，我们使用最先进的人脸识别网络计算了合成回放样本与原始训练图像之间的全局特征相似度。如表~\ref{tab:privacy_gen} 所示，由 ArcFace 和 CosFace 提取的跨身份相似度极低，表现出接近于零的均值和微小的方差。尽管以 15.36 的 FID 分数保持了较高的生成保真度，生成模型通过学习底层的数据结构分布而不是死记硬背显式的训练样本，成功地合成了全新的身份。这有力地证实了我们的生成式回放框架从根本上消除了身份泄露的风险，为增量深度伪造检测提供了一种高度安全的演练机制。

\section{Conclusion}
In this paper, we present Dual Confusion-Aware REgularization (Dual-CARE), a framework for enhancing generative replay in incremental face forgery detection. We analyze domain confusion between replay generators and new forgery models, identifying domain-safe samples for direct supervision and domain-risky samples that require adaptive handling. Guided by a Domain Confusion Score (DC Score), Dual-CARE dual-modulates generator updates and detector supervision, applying a Relative Separation Loss to domain-risky samples to balance informative cues and potential confusion. Extensive experiments show that Dual-CARE improves robustness and accuracy across diverse generative replay settings, while mitigating the negative impact of domain overlap, validating its effectiveness for incremental learning under evolving forgery threats.



==> ECCV_2026_Paper_Template/tab/Generation_analysis.tex <==
% \begin{table*}[h]
% \centering
% \caption{Performance comparison of various generative replay strategies on Protocol 1. We evaluate Full Replay, Fake-Only Replay, our dynamic Dual-CARE, and two fixed-alpha baselines.}
% \footnotesize
% \setlength{\tabcolsep}{4pt}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l@{\hspace{3pt}} c | c c c c c c c c | c c c c}
% \toprule
% % ---------------- Header (Row 1) ----------------
% \multirow{2}{*}{Method} & \multirow{2}{*}{Task} & \multicolumn{8}{c|}{Task-Incremental Performance (AUC)} & \multicolumn{4}{c}{Average Accuracy (ACC)} \\

% % ---------------- Header (Row 2) ----------------
% \cmidrule(lr){3-10} \cmidrule(lr){11-14}
% & & LDM & DFDCP & SDv21 & DDPM & DiT & CDF & Avg. & PD $\downarrow$ & Real & PD $\downarrow$ & Fake & PD $\downarrow$ \\
% \toprule

% % ---------------- Lower Bound ----------------
% \multirow{6}{*}{Lower Bound}
% & T1 & 99.99 & - & - & - & - & - & 99.99 & - & 99.85 & - & 99.90 & - \\
% & T2 & 80.75 & 88.76 & - & - & - & - & 84.76 & 15.23 & 87.80 & 12.05 & 45.63 & 54.27 \\
% & T3 & 77.46 & 52.63 & 99.99 & - & - & - & 76.69 & 23.30 & 99.60 & 0.25 & 36.55 & 63.35 \\
% & T4 & 35.18 & 55.52 & 31.75 & 99.93 & - & - & 55.60 & 44.39 & 89.41 & 10.44 & 35.39 & 64.51 \\
% & T5 & 51.44 & 50.77 & 70.63 & 77.10 & 99.21 & - & 69.83 & 30.16 & 89.00 & 10.85 & 37.62 & 62.28 \\
% & T6 & 52.73 & 80.54 & 81.78 & 50.34 & 53.30 & 99.56 & 69.71 & 30.28 & 89.51 & 10.34 & 41.28 & 58.62 \\
% \midrule

% % ---------------- Method A ----------------
% \multirow{6}{*}{Full Replay}
% & T1 & 99.99 & - & - & - & - & - & 99.99 & - & 99.70 & - & 99.85 & - \\
% & T2 & 99.68 & 90.63 & - & - & - & - & 95.16 & 4.83 & 82.47 & 17.23 & 92.44 & 7.41 \\
% & T3 & 99.19 & 89.04 & 99.94 & - & - & - & 96.06 & 3.93 & 97.37 & 2.33 & 83.70 & 16.15 \\
% & T4 & 90.90 & 86.37 & 99.65 & 99.98 & - & - & 94.23 & 5.76 & \textbf{98.80} & \textbf{0.90} & 67.63 & 32.22 \\
% & T5 & 94.59 & 84.95 & 98.01 & 93.73 & 99.21 & - & 94.10 & 5.89 & 88.42 & 11.28 & \textbf{88.09} & \textbf{11.76} \\
% & T6 & 96.59 & 84.61 & 94.96 & 98.08 & 75.67 & 99.37 & 91.55 & 8.44 & 84.55 & 15.15 & 83.96 & 15.89 \\
% \midrule

% % ---------------- Method B ----------------
% \multirow{6}{*}{Fake-Only Replay}
% & T1 & 99.99 & - & - & - & - & - & 99.99 & - & 99.75 & - & 99.90 & - \\
% & T2 & 95.74 & 90.51 & - & - & - & - & 93.13 & 6.86 & 71.42 & 28.33 & \textbf{95.18} & \textbf{4.72} \\
% & T3 & 96.00 & 77.23 & 99.98 & - & - & - & 91.07 & 8.92 & 73.63 & 26.12 & \textbf{93.05} & \textbf{6.85} \\
% & T4 & 97.99 & 75.01 & 98.90 & 99.94 & - & - & 92.96 & 7.03 & 76.85 & 22.90 & 83.41 & 16.49 \\
% & T5 & 97.49 & 55.68 & 98.65 & 78.56 & 99.12 & - & 85.90 & 14.09 & 58.20 & 41.55 & 78.82 & 21.08 \\
% & T6 & 95.39 & 76.24 & 98.09 & 49.94 & 52.10 & 99.63 & 78.56 & 21.43 & 82.77 & 16.98 & 63.10 & 36.80 \\
% \midrule

% % ---------------- alpha 0.5 ----------------
% \multirow{6}{*}{Fixed $s_t=0.5$}
% & T1 & 99.99 & - & - & - & - & - & 99.99 & - & 99.80 & - & 99.85 & - \\
% & T2 & 99.55 & 91.69 & - & - & - & - & 95.62 & 4.37 & 85.77 & 14.03 & 83.65 & 16.20 \\
% & T3 & 98.26 & 95.18 & 99.98 & - & - & - & 97.81 & 2.18 & \textbf{99.58} & \textbf{0.22} & 72.84 & 27.01 \\
% & T4 & 97.21 & 93.83 & 96.90 & 99.99 & - & - & 96.98 & 3.01 & 92.98 & 6.82 & 87.14 & 12.71 \\
% & T5 & 90.82 & 86.24 & 96.40 & 98.21 & 99.79 & - & 94.29 & 5.70 & 94.26 & 5.54 & 81.46 & 18.39 \\
% & T6 & 99.77 & 87.57 & 97.25 & 99.40 & 78.66 & 99.70 & 93.72 & 6.27 & 94.44 & 5.36 & 62.36 & 37.49 \\
% \midrule

% % ---------------- alpha 0.1 ----------------
% \multirow{6}{*}{Fixed $s_t=0.1$}
% & T1 & 99.99 & - & - & - & - & - & 99.99 & - & 99.90 & - & 99.90 & - \\
% & T2 & 99.84 & 91.10 & - & - & - & - & 95.47 & 4.52 & 88.57 & 11.33 & 86.58 & 13.32 \\
% & T3 & 99.72 & 95.33 & 99.93 & - & - & - & \textbf{98.32} & \textbf{1.67} & 98.18 & 1.72 & 85.22 & 14.68 \\
% & T4 & 97.42 & 95.07 & 96.33 & 99.99 & - & - & 97.20 & 2.79 & 96.81 & 3.09 & 77.26 & 22.64 \\
% & T5 & 92.19 & 87.73 & 97.65 & 94.80 & 98.94 & - & 94.26 & 5.73 & 94.92 & 4.98 & 77.28 & 22.62 \\
% & T6 & 99.59 & 88.71 & 96.69 & 98.86 & 75.19 & 99.69 & 93.12 & 6.87 & \textbf{95.38} & \textbf{4.52} & 61.39 & 38.51 \\
% \midrule

% % ---------------- Method C ----------------
% \multirow{6}{*}{\textbf{Ours (Adaptive)}}
% & T1 & 99.99 & - & - & - & - & - & 99.99 & - & 99.85 & - & 99.85 & - \\
% & T2 & 99.90 & 91.50 & - & - & - & - & \textbf{95.70} & \textbf{4.29} & \textbf{91.01} & \textbf{8.84} & 87.54 & 12.31 \\
% & T3 & 99.78 & 95.01 & 99.96 & - & - & - & 98.25 & 1.74 & 98.75 & 1.10 & 83.89 & 15.96 \\
% & T4 & 98.95 & 92.73 & 97.41 & 99.99 & - & - & \textbf{97.27} & \textbf{2.72} & 96.67 & 3.18 & \textbf{89.51} & \textbf{10.34} \\
% & T5 & 98.62 & 85.14 & 97.40 & 97.62 & 99.24 & - & \textbf{95.60} & \textbf{4.39} & \textbf{98.90} & \textbf{0.95} & 66.11 & 33.74 \\
% & T6 & 99.69 & 89.07 & 98.39 & 99.47 & 88.29 & 99.51 & \textbf{95.74} & \textbf{4.25} & 89.60 & 10.25 & \textbf{85.29} & \textbf{14.56} \\

% \bottomrule
% \end{tabular}}
% \label{tab:Generation analysis}
% \end{table*}

\begin{table*}[t]
\centering
\caption{Performance comparison of various generative replay strategies on Protocol 1. We evaluate Full Replay, Fake-Only Replay, our dynamic Dual-CARE, and two baselines with fixed confusion score .}
\footnotesize
\setlength{\tabcolsep}{4pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{l | c c c c c c c c | c c c c}
\toprule
% ---------------- Header (Row 1) ----------------
\multirow{2}{*}{Method} & \multicolumn{8}{c|}{Task-Incremental Performance (AUC)} & \multicolumn{4}{c}{Average Accuracy (ACC)} \\

% ---------------- Header (Row 2) ----------------
\cmidrule(lr){2-9} \cmidrule(lr){10-13}
& LDM & DFDCP & SDv21 & DDPM & DiT & CDF & Avg. & PD $\downarrow$ & Real & PD $\downarrow$ & Fake & PD $\downarrow$ \\
\toprule

% ---------------- Methods ----------------
Lower Bound & 52.73 & 80.54 & 81.78 & 50.34 & 53.30 & 99.56 & 69.71 & 30.28 & 89.51 & 10.34 & 41.28 & 58.62 \\
Full Replay & 96.59 & 84.61 & 94.96 & 98.08 & 75.67 & 99.37 & 91.55 & 8.44 & 84.55 & 15.15 & 83.96 & 15.89 \\
Fake-Only Replay & 95.39 & 76.24 & 98.09 & 49.94 & 52.10 & 99.63 & 78.56 & 21.43 & 82.77 & 16.98 & 63.10 & 36.80 \\
Fixed $s_t=0.5$ & 99.77 & 87.57 & 97.25 & 99.40 & 78.66 & 99.70 & 93.72 & 6.27 & 94.44 & 5.36 & 62.36 & 37.49 \\
Fixed $s_t=0.1$ & 99.59 & 88.71 & 96.69 & 98.86 & 75.19 & 99.69 & 93.12 & 6.87 & \textbf{95.38} & \textbf{4.52} & 61.39 & 38.51 \\
\textbf{Ours (Adaptive)} & 99.69 & 89.07 & 98.39 & 99.47 & 88.29 & 99.51 & \textbf{95.74} & \textbf{4.25} & 89.60 & 10.25 & \textbf{85.29} & \textbf{14.56} \\

\bottomrule
\end{tabular}}
\label{tab:Generation analysis}
\end{table*}

==> ECCV_2026_Paper_Template/tab/ablation.tex <==
% \begin{table}[h!]
% \centering
% \caption{Ablation study (AUC) on core components and distance metrics. Results are evaluated using the final Protocol 1 model at T6 and reported for tasks T1–T5.}
% \footnotesize

% % --- 微调列间距 ---
% \setlength{\tabcolsep}{3pt}

% % --- 微调行高 ---
% \renewcommand{\arraystretch}{1.2}

% \begin{tabular}{l ccccccc}
% \hline
% % ---------------- 表头 ----------------
% Variant & LDM & DFDCP & SDv21 & DDPM & DiT & CDF & Avg. \\
% \hline

% % ---------------- 组件消融 ----------------
% w/o DC-guided Gen & 95.42 & 83.61 & 94.16 & \textbf{96.38} & 94.99 & 99.21 & 93.96 \\
% w/o Gen-Real Sup. & 59.05 & 83.93 & 91.91 & 95.64 & 79.59 & 98.50 & 84.77 \\
% w/o $\mathcal{L}_{rs}$ & 94.28 & 79.41 & 97.18 & 86.88 & 94.55 & \textbf{99.67} & 91.99 \\
% \hline

% % ---------------- 距离度量消融 ----------------
% DCS-Cos + RS-Cos & 94.24 & 81.02 & 96.06 & 89.83 & 92.97 & 99.22 & 92.22 \\
% DCS-L2 + RS-L2 & 94.06 & 83.41 & 96.37 & 91.71 & 96.02 & 99.21 & 93.46 \\
% DCS-Cos + RS-L2 & 97.64 & 83.77 & 97.32 & 89.21 & 95.09 & 99.57 & 93.76 \\
% \hline

% % ---------------- "Ours" 行 ----------------
% \textbf{Dual-CARE (Ours)} & \textbf{98.45} & \textbf{87.36} & \textbf{97.71} & 95.28 & \textbf{98.07} & 98.93 & \textbf{95.96} \\
% \hline

% \end{tabular}

% \label{tab:ablation}
% \end{table}

% \begin{table}[h!]
% \centering
% \caption{Ablation study (AUC) on core components and distance metrics.}

% % --- 微调行高 ---
% \renewcommand{\arraystretch}{1.2}

% % 使用 resizebox 强制将表格宽度限制在文本宽度 (\textwidth) 内
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l cccccccc}
% \hline
% % ---------------- 表头 ----------------
% Variant & LDM & DFDCP & SDv21 & DDPM & DiT & CDF & Pre Avg. & Avg. \\
% \hline

% % ---------------- 组件消融 ----------------
% w/o DC-guided Gen & 95.42 & 83.61 & 94.16 & \textbf{96.38} & 94.99 & 99.21 & 92.91 & 93.96 \\
% w/o Gen-Real Sup. & 59.05 & 83.93 & 91.91 & 95.64 & 79.59 & 98.50 & 82.02 & 84.77 \\
% w/o $\mathcal{L}_{rs}$ & 94.28 & 79.41 & 97.18 & 86.88 & 94.55 & \textbf{99.67} & 90.46 & 91.99 \\
% \hline

% % ---------------- 距离度量消融 ----------------
% DCS-Cos + RS-Cos & 94.24 & 81.02 & 96.06 & 89.83 & 92.97 & 99.22 & 90.82 & 92.22 \\
% DCS-L2 + RS-L2 & 94.06 & 83.41 & 96.37 & 91.71 & 96.02 & 99.21 & 92.31 & 93.46 \\
% DCS-Cos + RS-L2 & 97.64 & 83.77 & 97.32 & 89.21 & 95.09 & 99.57 & 92.61 & 93.76 \\
% \hline

% % ---------------- "Ours" 行 ----------------
% \textbf{Dual-CARE (Ours)} & \textbf{98.45} & \textbf{87.36} & \textbf{97.71} & 95.28 & \textbf{98.07} & 98.93 & \textbf{95.37} & \textbf{95.96} \\
% \hline

% \end{tabular}
% } % 注意这里是 resizebox 的右括号

% \label{tab:ablation}
% \end{table}

\begin{table}[h!]
\centering
\caption{Ablation study (AUC) on core components and distance metrics. Results are evaluated using the final Protocol 1 model at T6 and reported for tasks T1–T5.}
\footnotesize

% --- 微调列间距 ---
\setlength{\tabcolsep}{3pt}

% --- 微调行高 ---
\renewcommand{\arraystretch}{1.2}

\begin{tabular}{l cccccc}
\hline
% ---------------- 表头 ----------------
Variant & LDM & DFDCP & SDv21 & DDPM & DiT & Avg. \\
\hline

% ---------------- 组件消融 (修正命名) ----------------

w/o DC-guided Gen & 95.42 & 83.61 & 94.16 & 96.38 & \textbf{94.99} & 92.91 \\
\hline


w/o Gen-Real Sup. & 88.41 & 79.17 & 98.52 & 52.04 & 53.47 & 74.32 \\
w/o $\mathcal{L}_{rs}$ & 92.75 & 89.29 & \textbf{99.34} & 90.47 & 83.04 & 90.97 \\
\hline

% ---------------- 距离度量消融 (修正命名) ----------------
DCS-Cos + RS-Cos & 97.96 & \textbf{92.59} & 97.52 & 98.2 & 74.02 & 92.05 \\
DCS-L2 + RS-L2 & \textbf{99.77} & 85.62 & 96.09 & 97.12 & 79.1 & 91.54 \\
DCS-Cos + RS-L2 & 99.54 & 86.37 & 97.31 & 99.28 & 82.05 & 92.91 \\
\hline

% ---------------- "Ours" 行 ----------------
\textbf{Dual-CARE (Ours)} & 99.69 & 89.07 & 98.39 & \textbf{99.47} & 88.29 & \textbf{94.98} \\
\hline

\end{tabular}


\label{tab:ablation}
\end{table}

==> ECCV_2026_Paper_Template/tab/alpha_p1.tex <==
\begin{table*}[h!]
\centering
\caption{Ablation study of normalization functions for the DC Score ($\alpha$) under Protocol 1.}
\footnotesize
\begin{tabular}{l@{\hspace{3pt}} c | c c c c c c c c}
\toprule
Method & Task & LDM & DFDCP & SDv21 & DDPM & DiT & CDF & Avg. & $\alpha$ \\
\toprule

% ================== OURS tanh ==================
\multirow{6}{*}{tanh}
& T1 & 99.99 & - & - & - & - & - & 99.99 & - \\
& T2 & 99.90 & 91.50 & - & - & - & - & 95.70 & 93.86 \\
& T3 & 99.78 & 95.01 & 99.96 & - & - & - & 98.25 & 99.82 \\
& T4 & 98.95 & 92.73 & 97.41 & 99.99 & - & - & 97.27 & 25.99 \\
& T5 & 98.62 & 85.14 & 97.40 & 97.62 & 99.24 & - & 95.60 & 93.25 \\
& T6 & 99.69 & 89.07 & 98.39 & 99.47 & 88.29 & 99.51 & 95.74 & 99.36 \\
\midrule

% ================== sigmoid ==================
\multirow{6}{*}{sigmoid}
& T1 & 99.99 & - & - & - & - & - & 99.99 & - \\
& T2 & 99.94 & 90.98 & - & - & - & - & 95.46 & 82.49 \\
& T3 & 99.91 & 94.89 & 99.92 & - & - & - & 98.24 & 98.15 \\
& T4 & 99.04 & 93.40 & 98.77 & 99.99 & - & - & 97.80 & 74.07 \\
& T5 & 98.36 & 90.01 & 94.45 & 97.82 & 96.72 & - & 95.47 & 77.36 \\
& T6 & 92.79 & 87.27 & 96.59 & 99.49 & 85.42 & 99.60 & 93.53 & 92.20 \\
\midrule

% ================== d/5 ==================
\multirow{6}{*}{d/5}
& T1 & 99.99 & - & - & - & - & - & 99.99 & - \\
& T2 & 99.93 & 91.72 & - & - & - & - & 95.82 & 30.91 \\
& T3 & 99.50 & 94.49 & 99.88 & - & - & - & 97.96 & 64.22 \\
& T4 & 92.24 & 92.68 & 95.89 & 99.99 & - & - & 95.20 & 6.05 \\
& T5 & 92.20 & 92.31 & 95.77 & 97.37 & 98.76 & - & 95.28 & 19.47 \\
& T6 & 99.83 & 89.18 & 97.59 & 97.50 & 81.33 & 99.60 & 94.17 & 41.76 \\

\bottomrule
\end{tabular}

\label{tab:alpha_p1}
\end{table*}

==> ECCV_2026_Paper_Template/tab/alpha_p2.tex <==
\begin{table}[h]
\centering
\footnotesize
\caption{Performance comparison of normalization functions under Protocol 2.}
\setlength{\tabcolsep}{3.0pt} % 稍微减小列间距以容纳新增的一列
\begin{tabular}{l@{\hspace{3pt}} c | c c c c c c}
\toprule
% ---------------- 表头 ----------------
Method & Task & DDPM & FF++ & DFDCP & CDF & Avg. & $s_t$ \\
\toprule

% ---------------- OURS (Avg. 已加粗) ----------------
\multirow{4}{*}{tanh} 
& T1 & 99.99 & - & - & - & 99.99 &\\
& T2 & 99.88 & 94.51 & - & - & 97.20 & 0.9997\\
& T3 & 99.60 & 89.28 & 91.97 & - & 93.62 & 0.9999\\
& T4 & 98.87 & 85.90 & 92.04 & 98.12 & 93.73 & 0.9769\\
\midrule
% ---------------- sigmoid ----------------
\multirow{4}{*}{sigmoid}
& T1 & 99.99 & - & - & - & 99.99 & - \\
& T2 & 97.99 & 94.97 & - & - & 96.48 & 0.9875 \\
& T3 & 98.41 & 88.29 & 89.79 & - & 92.16 & 0.9971 \\
& T4 & 98.83 & 79.24 & 89.23 & 98.88 & 91.54 & 0.9013 \\
\midrule

% ---------------- d/5 ----------------
\multirow{4}{*}{d/5}
& T1 & 99.99 & - & - & - & 99.99 & - \\
& T2 & 98.55 & 94.97 & - & - & 96.76 & 0.8077 \\
& T3 & 99.86 & 86.25 & 91.13 & - & 92.41 & 0.9999 \\
& T4 & 99.91 & 77.91 & 90.41 & 98.47 & 91.67 & 0.4694 \\

\bottomrule
\end{tabular}
\label{tab:alpha_p2}  
\end{table}

==> ECCV_2026_Paper_Template/tab/p1.tex <==
\begin{table*}[t]
\centering
\caption{Quantitative comparison (AUC) on Protocol 1 (Mixed-Era Forgery Incremental). L-Bound (Lower Bound) denotes vanilla incremental learning. Task 1 (T1) to Task 6 (T6) represent the incremental steps in the dataset sequence. Pre Avg. denotes the average performance over all previous tasks, excluding the current task. PD $\downarrow$ denotes the Performance Dropping rate. Bests are marked with \textbf{bold}.}
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{l @{\hspace{3pt}}c c  |c c c c c c  |c c c}
\toprule
% ---------------- 表头 (单行) ----------------
Method & Venue & Task & LDM & DFDCP & SDv21 & DDPM & DiT & CDF & Pre Avg. & Avg. & PD $\downarrow$ \\
\toprule

% ---------------- Lower Bound ----------------
\multirow{6}{*}{L-Bound} & \multirow{6}{*}{--} & T1 & 99.99 & - & - & - & - & - & - & 99.99 & - \\
& & T2 & 80.75 & 88.76 & - & - & - & - & 80.75 & 84.76 & 15.23 \\
& & T3 & 77.46 & 52.63 & \textbf{99.99} & - & - & - & 65.04 & 76.69 & 23.30 \\
& & T4 & 35.18 & 55.52 & 31.75 & 99.93 & - & - & 40.81 & 55.60 & 44.39 \\
& & T5 & 51.44 & 50.77 & 70.63 & 77.10 & 99.21 & - & 62.48 & 69.83 & 30.16 \\
& & T6 & 52.73 & 80.54 & 81.78 & 50.34 & 53.30 & \textbf{99.56} & 63.73 & 69.71 & 30.28 \\
\midrule

% ---------------- 中间的单行方法 ----------------
LwF & TPAMI' 17 & T6 & 81.31 & 78.16 & 89.40 & 49.11 & 76.92 & 98.15 & 74.98 & 78.84 & 21.15 \\
iCaRL & CVPR' 17 & T6 & 83.72 & 76.31 & 84.54 & 59.75 & 71.91 & 99.20 & 75.25 & 81.39 & 18.60 \\
DER & CVPR' 21 & T6 & 77.31 & 80.12 & 90.36 & 82.01 & 83.23 & 99.07 & 82.61 & 84.24 & 15.75 \\
CoReD & MM' 21 & T6 & 88.58 & 83.79 & 94.97 & 78.79 & 71.32 & 99.17 & 83.49 & 82.47 & 17.52 \\
HDP & IJCV' 24 & T6 & 94.31 & 85.82 & 93.73 & 95.10 & 81.53 & 99.40 & 90.10 & 83.96 & 16.03 \\
\midrule

% ---------------- DFIL ----------------
\multirow{6}{*}{DFIL} & \multirow{6}{*}{MM' 23} & T1 & 99.99 & - & - & - & - & - & - & 99.99 & - \\
& & T2 & 97.22 & 91.07 & - & - & - & - & 97.22 & 94.14 & 5.85 \\
& & T3 & 98.23 & 75.91 & 99.98 & - & - & - & 87.07 & 91.37 & 8.62 \\
& & T4 & 94.01 & 72.43 & 99.80 & \textbf{99.98} & - & - & 88.75 & 91.56 & 8.43 \\
& & T5 & 95.84 & 66.56 & 98.61 & 88.32 & 96.31 & - & 87.33 & 89.13 & 10.86 \\
& & T6 & 92.37 & 73.39 & 99.02 & 84.27 & 77.39 & 99.48 & 85.29 & 87.66 & 12.33 \\
\midrule

% ---------------- SUR-LID ----------------
\multirow{6}{*}{SUR-LID} & \multirow{6}{*}{CVPR' 25} & T1 & 99.99 & - & - & - & - & - & - & 99.99 & - \\
& & T2 & 99.31 & 90.32 & - & - & - & - & \textbf{99.31} & 94.82 & 5.17 \\
& & T3 & 99.17 & 87.95 & 99.96 & - & - & - & 93.56 & 95.69 & 4.30 \\
& & T4 & \textbf{99.50} & 80.27 & 99.54 & 99.73 & - & - & 93.10 & 94.76 & 5.23 \\
& & T5 & 98.70 & 75.11 & \textbf{99.62} & \textbf{99.89} & \textbf{99.55} & - & 93.33 & 94.58 & 5.41 \\
& & T6 & 97.40 & 82.18 & \textbf{99.03} & \textbf{98.35} & 92.50 & 99.22 & 93.89 & 94.78 & 5.21 \\
\midrule

% ---------------- OURS ----------------
\multirow{6}{*}{\textbf{Dual-CARE (Ours)}} & \multirow{6}{*}{--} & T1 & 99.99 & - & - & - & - & - & - & 99.99 & - \\
& & T2 & \textbf{99.67} & \textbf{91.50} & - & - & - & - & 95.58 & \textbf{95.58} & \textbf{4.41} \\
& & T3 & \textbf{99.60} & \textbf{91.78} & 99.97 & - & - & - & \textbf{97.12} & \textbf{97.12} & \textbf{2.87} \\
& & T4 & 93.63 & \textbf{90.91} & 99.25 & \textbf{99.98} & - & - & \textbf{95.94} & \textbf{95.94} & \textbf{4.05} \\
& & T5 & \textbf{99.08} & \textbf{86.96} & \textbf{99.62} & 96.45 & 95.59 & - & \textbf{95.54} & \textbf{95.54} & \textbf{4.45} \\
& & T6 & \textbf{98.45} & \textbf{87.36} & 97.71 & 95.28 & \textbf{98.07} & 98.93 & \textbf{95.37} & \textbf{95.96} & \textbf{4.03} \\

\bottomrule
\end{tabular}}
\label{tab:main_comparison}
\end{table*}

==> ECCV_2026_Paper_Template/tab/p2.tex <==
\begin{table}[h!]
\centering
\caption{Quantitative comparison (AUC) on Protocol 2. L-Bound denotes vanilla incremental learning without any strategy. }
\footnotesize
         \setlength{\tabcolsep}{3.7pt} 
\begin{tabular}{l@{\hspace{3pt}}  c | c c c c c} 
\toprule
% ---------------- 表头 (单行) ----------------
Method & Task & DDPM & FF++ & DFDCP & CDF & Avg. \\ 
\toprule

% ---------------- Lower Bound ----------------
\multirow{4}{*}{L-Bound} 
& T1 & 99.99 & - & - & - & 99.99 \\
& T2 & 69.60 & 95.16 & - & - & 82.38 \\
& T3 & 60.58 & 71.28 & 92.38 & - & 74.75 \\
& T4 & 53.39 & 65.92 & 82.23 & 99.77 & 75.33 \\
\midrule

% ---------------- LwF ----------------
\multirow{4}{*}{LwF} 
& T1 & 99.99 & - & - & - & 99.99 \\
& T2 & 81.01 & 85.02 & - & - & 83.02 \\
& T3 & 76.12 & 65.07 & 93.91 & - & 78.37 \\
& T4 & 61.71 & 61.14 & 81.35 & 98.18 & 75.60 \\
\midrule

% ---------------- iCaRL ----------------
\multirow{4}{*}{iCaRL} 
& T1 & 99.99& - & - & - & 99.99 \\
& T2 & 96.56 & 91.02 & - & - & 93.79 \\
& T3 & 91.71 & 80.07 & 90.95 & - & 87.58 \\
& T4 & 91.79 & 73.93 & 87.10 & 99.09 & 87.98 \\
\midrule

% ---------------- DFIL ----------------
\multirow{4}{*}{DFIL} 
& T1 & 99.99 & - & - & - & 99.99 \\
& T2 & 97.17 & 93.31 & - & - & 95.24 \\
& T3 & 93.51 & 71.27 & 91.64 & - & 85.47 \\
& T4 & 92.33 & 68.10 & 80.74 & 99.63 & 85.20 \\
\midrule

% ---------------- SUR-LID (Avg. 已加下划线) ----------------
\multirow{4}{*}{SUR-LID} 
& T1 & 99.99 & - & - & - & 99.99 \\
& T2 & 99.35 & 92.36 & - & - & 95.85 \\
& T3 & 99.13 & 81.51 & 92.13 & - & 90.92 \\
& T4 & 98.16 & 78.16 & 86.37 & 99.18 & 90.47 \\
\midrule

% ---------------- OURS (Avg. 已加粗) ----------------
\multirow{4}{*}{\textbf{Dual-CARE (Ours)}} 
& T1 & 99.99 & - & - & - & 99.99 \\
& T2 & 99.88 & 94.51 & - & - & \textbf{97.20} \\
& T3 & 99.60 & 89.28 & 91.97 & - & \textbf{93.62} \\
& T4 & 98.87 & 85.90 & 92.04 & 98.12 & \textbf{93.73} \\

\bottomrule
\end{tabular}
\label{tab:p2_comparison}
\end{table}
